Automatic Static Bug Detection for Machine Learning Libraries: Are We There Yet?

Automatic detection of software bugs is a critical task in software security. Many static tools that can help detect bugs have been proposed. While these static bug detectors are mainly evaluated on general software projects call into question their practical effectiveness and usefulness for machine learning libraries. In this paper, we address this question by analyzing five popular and widely used static bug detectors, i.e., Flawfinder, RATS, Cppcheck, Facebook Infer, and Clang static analyzer on a curated dataset of software bugs gathered from four popular machine learning libraries including Mlpack, MXNet, PyTorch, and TensorFlow with a total of 410 known bugs. Our research provides a categorization of these tools' capabilities to better understand the strengths and weaknesses of the tools for detecting software bugs in machine learning libraries. Overall, our study shows that static bug detectors find a negligible amount of all bugs accounting for 6/410 bugs (0.01%), Flawfinder and RATS are the most effective static checker for finding software bugs in machine learning libraries. Based on our observations, we further identify and discuss opportunities to make the tools more effective and practical.

==> sec/results/rq2.tex <==
\subsection{RQ2: Effectiveness of Automatic Mapping Techniques}

% \song{diff and fixed-warning report totally different matches?} \nima{They share 4 true mappings}

Table~\ref{tab:mappingPerf} shows the number of correct matching over the total number of matching for each automatic mapping technique distributed over the studied ML libraries. In general, using the automatic mapping techniques, the four static vulnerability detectors only detect 3 unique bugs. As shown in this table, the diff-based mapping approach could detect 6 correct vulnerability candidates while the fix-based mapping method could only detect 4 vulnerability candidates. The result is consistent with previous studies~\cite{tomassi2021real, habib2018many}, i.e., the diff mapping technique outperforms the fixed-warning technique regarding identifying vulnerability candidates. As previously mentioned, the fixed-warning-based technique discovers vulnerability candidates by keyword matching and a set of heuristic rules built as regular expressions using information from the commits characteristics, e.g., message and title. As a result, if developers put more effort into giving more meaningful information about bugs in commits, the accuracy of the fixed technique increases. 

\begin{tcolorbox}
\textbf{Finding 2:} Diff-based mapping technique outperforms the fixed-warning-based approach on the studied six ML libraries regarding the number of correctly matched vulnerability candidates. 
\end{tcolorbox}

% [width=8.5cm,
% outer arc=0mm,
% inner arc=0mm,
%                   enhanced,
%                   frame hidden,
%                   interior hidden,
%                   boxsep=0pt,
%                   left=3pt,
%                   right=3pt,
%                   top=3pt,
%                   ]

\input{tables/mapping_table}


==> tables/mapping_table.tex <==
\begin{table}[t!]
\centering
\caption{Total number of vulnerability candidates reported by each automatic mapping technique distributed over static detectors. We show the number of correct mappings / the total number of mappings. The last column shows the overall number of matching. The number inside the parenthesis indicates the total number of unique real-world ML vulnerabilities detected. }
\label{tab:mappingPerf}
\renewcommand{\arraystretch}{1}
\begin{tabular}{|c|c|c|c|}
\hline
\multirow{2}{*}{Static Detector} & \multicolumn{2}{|c|}{Mapping technique} & 
\multirow{2}{*}{Overall} \\
\cline{2-3}
           & Diff & Fixed &        \\
\hline
Flawfinder & 0/20 & 0/23  & 0/43     \\
\hline
RATS       & 1/14 & 0/7   & 1/21      \\
\hline
Cppcheck   & 5/8  & 4/11  & 9/19      \\
\hline
Infer      & 0/20 & 0/7   & 0/27     \\
\hline
Overall    & 6/62 & 4/48  & 10(3) \\
\hline
\end{tabular}%
\end{table}
